Active Simultaneously Transmitting and Reflecting (STAR)-RISs: Modelling and Analysis

A hardware model for active simultaneously transmitting and reflecting reconfigurable intelligent surfaces (STAR-RISs) is proposed consisting of reflection-type amplifiers. The amplitude gains of the STAR element are derived for both coupled and independent phase-shift scenarios. Based on the proposed hardware model, an active STAR-RIS-aided two-user downlink communication system is investigated. Closed-form expressions are obtained for the outage probabilities of both the coupled and independent phase-shift scenarios. To obtain further insights, scaling laws and diversity orders are derived for both users. Analytical results confirm that active STAR-RIS achieves the same diversity orders as passive ones while their scaling laws are different. It is proved that average received SNRs scale with M and M^2 for active and passive STAR-RISs, respectively. Numerical results show that active STAR-RISs outperform passive STAR-RISs in terms of outage probability especially when the number of elements is small.

==> others.tex <==
In terms of energy consumption, a STAR-RIS can be passive lossy, passive lossless or active.
Under dual-sided incidence~\cite{dual}, each STAR element has four T\&R coefficients, i.e., $\Tilde{R}^A_m$, $\Tilde{R}^B_m$, $\Tilde{T}^{AB}_m$, and $\Tilde{R}^{BA}_m$. These four coefficients transform the incident signals to the output signals of each STAR element. The relation between the incident and output signals is given by:
\vspace{-0.1in}
\begin{equation}\label{tr_def}
    \begin{pmatrix}
y^A_m\\
y^B_m
\end{pmatrix} =
    \begin{pmatrix}
\Tilde{R}^A_m & \Tilde{T}^{AB}_m\\
\Tilde{T}^{BA}_m & \Tilde{R}^B_m
\end{pmatrix}
\begin{pmatrix}
s^A_m\\
s^B_m
\end{pmatrix},
\end{equation}
or equivalently, $\mathbf{y}_m = \mathbf{\Xi}_m \cdot \mathbf{s}_m$, where $\mathbf{\Xi}_m$ is the T\&R matrix of the $m$th STAR element. According to microwave network analysis, a STAR element is passive lossless if $\mathbf{\Xi}_m$ is unitary, i.e., $\mathbf{\Xi}_m^H\mathbf{\Xi}_m = \mathbf{I}_2$, where $\mathbf{I}_2$ denotes the two-by-two identity matrix. For passive lossy STAR element, $\mathbf{\Xi}_m^H\mathbf{\Xi}_m \prec \mathbf{I}_2$, and for active STAR element, $\mathbf{\Xi}_m^H\mathbf{\Xi}_m \succ \mathbf{I}_2$~\cite{pozar2011microwave}.
%
In terms of reciprocity, a STAR-RIS can be either reciprocal or nonreciprocal. A STAR element is reciprocal if the T\&R matrix $\mathbf{\Xi}_m$ is symmetrical, i.e., $\Tilde{T}^{AB}_m = \Tilde{T}^{BA}_m$. For nonreciprocal STAR matrix, we have $\Tilde{T}^{AB}_m \neq \Tilde{T}^{BA}_m$. 
%For application scenarios where all users under service are located on one side of the STAR-RIS (for example, \textit{side A}), signal power is lost if $\Tilde{T}^{BA}_m \neq 0$ even if all the STAR element might be lossless. An nonreciprocal STAR element is ideal in these scenarios to avoid power leakage from \textit{side A} to \textit{side B}. 
In the letter, we focus on hardware models for active STAR-RISs with reciprocal elements where both independent and coupled phase-shift scenarios are considered.

\section{Mac Control}
\begin{figure}[h!]
    \begin{center}
        \includegraphics[scale=0.07]{mac_fig/MAC_RIS.jpg}
        \caption{STAR-RIS as a medium access controller for RF resources.}
        \label{sys1}
    \end{center}
\end{figure}
\begin{itemize}
    \item For wireless communications through the RF medium, there is a scarcity of medium access control. In today's communication system, transceivers of different applications shares the same physical transmission medium. Moreover, the medium is only divided into different cells based on physical distances or different frequency bands based on the carrier frequencies and bandwidths. However, due to the increased number or mobile devices, more and more terminals need to be accommodated within the urban area. In the same time, new wireless technologies are emerging which may take up more RF resource, such as RF sensing network for IoT, UAV local networks, and ...\\
    Consequently, there is a increasing need for a medium access controller to mitigate interference and collisions of the wireless channels.
\end{itemize}




%%%%%%%%%%
\begin{comment}
\begin{figure*}[t!]
\centering
\subfigure[Time-Switching]{\label{sysa}
\includegraphics[width= 2in]{mac_fig/sys_a.eps}}
\subfigure[Unicast]{\label{sysb}
\includegraphics[width= 2in]{mac_fig/sys_b.eps}}
\subfigure[Multicast]{\label{sysc}
\includegraphics[width= 2.2in]{mac_fig/sys_c.eps}}
\caption{Illustration of the working modes of the full-duplex STAR-RISs}\label{nice}
\end{figure*}

As shown in Fig.~\ref{sysa}, for the time-switching double-sided unicast scenario, Tx1 and Tx2 transmit their signals to their corresponding receivers in separate time slots. In the first time slot, Tx1 sends message $s_1$ to Rx1, and the $m$th element is configured to transmit $s_1$ from \textit{Space A} to \textit{Space B} with transmission coefficient $T^{A,B}_m$. Similarly, in the second time slot, $s_2$ is transmitted from \textit{Space B} to \textit{Space A} with transmission coefficient $T^{B,A}_m$. Because $s_1$ and $s_2$ are transmitted in different time slots, $T^{A,B}_m$ and $T^{B,A}_m$ can be independently configured. To sum up, we have the following signal model for STAR-RIS:
\subsubsection*{Case 1}
For the time-switching double-sided unicast scenario, the STAR-RIS elements can be modeled using the following transmission coefficients:
\begin{equation}
    T^{A,B}_m = \beta^{A,B}_m e^{j\phi^{A,B}_m} \text{, and  } T^{B,A}_m = \beta^{B,A}_m e^{j\phi^{B,A}_m},
\end{equation}
where $\beta^{A,B}_m$ and $\beta^{B,A}_m\in [0,1]$ are the amplitudes of the corresponding transmission coefficients, $\phi^{A,B}_m$ and $\phi^{B,A}_m \in[0,2\pi)$ are the phases of the transmission coefficients in time slot 1 and 2, respectively.
\end{comment}



%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
Different from the single source case which have been previously studied, the T\&R coefficients on the two sides of the $m$th element can be defined as follows:
\begin{align}\label{tab1}
    T^{A,B}_m &= ({E}^J+{E}^K_2+{E}^{inc}_1)/{E}^{inc}_1, \\
    T^{B,A}_m &= ({E}^J+{E}^K_1+{E}^{inc}_2)/{E}^{inc}_2, \\
    R^{A}_m &= ({E}^J+{E}^K_1+{E}^{inc}_2)/{E}^{inc}_1, \\ \label{rb1}
    R^{B}_m &= ({E}^J+{E}^K_2+{E}^{inc}_1)/{E}^{inc}_2,
\end{align}
where $E^J = ||\mathbf{E}^J||_2$,  $E^K_1 = ||\mathbf{E}^K_1||_2$, $E^K_2 = ||\mathbf{E}^K_2||_2$, $E^{inc}_1 = ||\mathbf{E}^{inc}_1||_2$, and $E^{inc}_2 = ||\mathbf{E}^{inc}_2||_2$ are the magnitudes of the corresponding electric field at the $m$th element. 

\begin{theorem}\label{t1}
Given incident signals on both sides ($E^{inc}_1$ and $E^{inc}_2$), a STAR-RIS element can be modeled using the following coefficients:
\begin{align}\label{tab}
    &T^{A,B}_m = T^0_m + \beta R^0_m,\\ \label{tba}
    &T^{B,A}_m = T^0_m + (1/\beta) R^0_m,\\ \label{ra}
    &R^{A}_m = R^0_m + \beta T^0_m,\\ \label{rb}
    &R^{B}_m = R^0_m + (1/\beta) T^0_m,
\end{align}
where $T^0_m = \frac{2Z_e}{2Z_e+\eta} - \frac{Z_m}{Z_m+2\eta}$, $R^0_m = \frac{Z_m}{Z_m+2\eta}-\frac{\eta}{2Z_e+\eta}$, $\eta$ is the free space wave impedance, and $\beta = E^{inc}_2/E^{inc}_1$ is the ratio between the amplitudes of the incident electric fields.
\begin{proof}
The boundary conditions~\cite{rNGfm99RfAqifzEoqjYY9NPszcDnpChRWu} of EM field at the surface can be expressed as $\hat{z}\times (\mathbf{H}^J_2-\mathbf{H}^J_1)\hat{y} = \mathbf{J}_s\hat{x}$ and $\hat{z}\times(\mathbf{E}^K_1 - \mathbf{E}^K_2)=\mathbf{K}_s\hat{y}$. Next, by considering \eqref{js} and \eqref{ks} with the boundary conditions, $E^J$ and $E^K_1$ in \eqref{tab1}-\eqref{rb1} can be expressed in terms of $Z_e$, $Z_m$, and $\eta$, i.e., we have the following:
\begin{align}\label{tab2}
    &E^J = \frac{-\eta(E^{inc}_1+E^{inc}_2)}{2Z_e+\eta},\\ \label{tab3}
    &E^K_1 = \frac{Z_m(E^{inc}_1-E^{inc}_2))}{Z_m+2\eta}.
\end{align}
Finally, by plugging \eqref{tab2} and \eqref{tab3} into \eqref{tab1}-\eqref{rb1}, the proof is finished.
\end{proof}
\end{theorem}

\begin{remark}
In \eqref{tab}-\eqref{rb}, $T^0_m$ and $R^0_m$ are the T\&R coefficients given a one-sided signal incidence. According to existing studies~\cite{xu_star,liu_star,mu_star}, the phases of $T^0_m$ and $R^0_m$, i.e., $\phi^T_m$ and $\phi^R_m$ can be independently configured while their amplitudes are constrained through the law of energy conservation, namely:
\begin{align}
    |T^0_m|^2+|R^0_m|^2 \leq 1\\
    \phi^T_m,\ \phi^R_m \in [0,2\pi).
\end{align}
For passive lossless STAR-RIS element, $\phi^T_m$ and $\phi^R_m$ are further correlated~\cite{xu_correlated}.
\end{remark}
The physical meaning of these coefficients can be understood through \eqref{tab}-\eqref{rb}: For general cases, $T^{A,B}_m \neq T^{B,A}$, and $R^A_m \neq R^B_m$. This is due to the asymmetric strengths of incident EM waves on the two sides. In the following, we present the signal models for STAR-RISs operating in purely transmitting, purely reflecting, and simultaneous transmitting and reflecting modes.
